Optimal Defaults, Limited Enforcement and the Regulation of Contracts

We study how governments promote social welfare through the design of contracting environments. We model the regulation of contracting as default delegation: the government chooses a delegation set of contract terms it is willing to enforce, and influences the default terms that serve as outside options in parties' negotiations. Our analysis shows that limiting the delegation set principally mitigates externalities, while default terms primarily achieve distributional objectives. Applying our model to the regulation of labor contracts, we derive comparative statics on the optimal default delegation policy. As equity concerns or externalities increase, in-kind support for workers increases (e.g. through benefits requirements and public health insurance). Meanwhile, when worker bargaining power decreases away from parity, support for workers increases in cash (e.g. through cash transfers and minimum wage laws).

==> mycommands.tex <==
%% ITEMIZE & ENUMERATE ENVIRONMENTS W/O BIG PARAGRAPH SKIPS
\usepackage{accents}
\setcounter{tocdepth}{2}

\newenvironment{itemize*}%
  {\begin{itemize}%
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{itemize}}
  
  \newenvironment{myquote}{%%
  \begin{itemize}[topsep=0pt]
  \item[]}{\end{itemize}}

\newenvironment{enumerate*}%
  {\begin{enumerate}%
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{enumerate}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{subcaption}

\usepackage[round]{natbib}
\bibliographystyle{aer}
\usepackage{sectsty} % For section format.
%% SECTION STUFF 
\sectionfont{\fontsize{13}{13}\selectfont}
\subsectionfont{\fontsize{11}{11}\selectfont}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}

% USEFUL SYMBOLS
\newcommand{\br}{\mathbf{br}}
\newcommand{\betaswf}{\beta\operatorname{-SWF}}
\newcommand{\Pj}{\mathbb{P}_j}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ee}{\mathcal{E}}
\newcommand{\yy}{\mathcal{Y}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\Gsp}{G^{SP}}
\newcommand{\starc}{\textbf{(*)}}
\newcommand{\myline}{\begin{center}\noindent\rule{8cm}{0.4pt}\end{center}}
\newcommand{\Var}{\mathbb{V}\text{ar}}
\newcommand{\Cov}{\text{Cov}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\newcommand{\ubar}[1]{\underline{#1}
\newcommand{\thetalow}{\ubar{\theta}}
\newcommand{\thetahi}{\bar{\theta}}
\newcommand{\nulow}{\ubar{\nu}}
\newcommand{\nuhi}{\bar{\nu}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\what}{\textcolor{red}{\textbf{(???)}}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\ctilde}{\tilde{c}}
\newcommand{\qwf}{q^{wf}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\qmin}{q^{\min}}
\newcommand{\qmax}{q^{\max}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\overline{q}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\qubar}{\underline{q}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\ytilde}{\tilde{y}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\ones}{\mathbf{1}}
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\bSigma}{\mathbf{\Sigma}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\MM}{\mathbf{M}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\Diff}{\operatorname{Diff}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\ql}{q_L}
\renewcommand{\d}{\text{d}}
\newcommand{\qh}{q_H}
\newcommand{\tl}{t_L}
\newcommand{\barcni}{\bar{c}_{-i}}
\newcommand{\cl}{c_L}
\newcommand{\cn}{c_N}
\newcommand{\bb}{\mathbf{b}}
\renewcommand{\th}{t_H}
\newcommand{\thetah}{\theta_H}
\newcommand{\C}{\mathcal{C}}
\newcommand{\thetal}{\theta_L}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\bxtilde}{\mathbf{\tilde{x}}}
\newcommand{\grad}{\nabla}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bep}{\boldsymbol{\epsilon}}
\newcommand{\mvpf}{\textsc{mvpf}}
\newcommand{\fe}{\textsc{fe}}
\newcommand{\wtp}{\textsc{wtp}}
\newcommand{\WS}{\operatorname{WS}}
\newcommand{\phat}{\hat{p}}
\newcommand{\vc}{\vec{c}}
\newcommand{\p}{\mathbf{p}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\SWF}{\operatorname{SWF}}
\newcommand{\default}{\text{default}}
\newcommand{\state}{\text{state }}




%% ENVIRONMENTS 
\newtheorem{theorem}{Theorem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{corollary}{Corollary}
\newtheorem{result}{Result}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{example}[definition]{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{assumption}[theorem]{Assumption}
\renewenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}


